Synthesizing Dominant Strategies for Liveness (Full Version)

Reactive synthesis automatically derives a strategy that satisfies a given specification. However, requiring a strategy to meet the specification in every situation is, in many cases, too hard of a requirement. Particularly in compositional synthesis of distributed systems, individual winning strategies for the processes often do not exist. Remorsefree dominance, a weaker notion than winning, accounts for such situations: dominant strategies are only required to be as good as any alternative strategy, i.e., they are allowed to violate the specification if no other strategy would have satisfied it in the same situation. The composition of dominant strategies is only guaranteed to be dominant for safety properties, though; preventing the use of dominance in compositional synthesis for liveness specifications. Yet, safety properties are often not expressive enough. In this paper, we thus introduce a new winning condition for strategies, called delay-dominance, that overcomes this weakness of remorsefree~dominance: we show that it is compositional for many safety and liveness specifications, enabling a compositional synthesis algorithm based on delay-dominance for general specifications. Furthermore, we introduce an automaton construction for recognizing delay-dominant strategies and prove its soundness and completeness. The resulting automaton is of single-exponential size in the squared length of the specification and can immediately be used for safraless synthesis procedures. Thus, synthesis of delay-dominant strategies is, as synthesis of winning strategies, in 2EXPTIME.

==> running_example.tex <==
\section{Running Example}\label{sec:running_example}

Throughout this paper, we use a simple running example to illustrate the introduced concepts.
Consider a system consisting of two system processes $p_1$ and $p_2$. Both processes can send a message to the other process and are able to receive messages from the other process. Hence, there are two variables $m_1$ and $m_2$ modeling the messages. For process $p_i$, variables $m_i$ is an output while variables $m_{1-i}$ is an input.
Both processes are required to send a message eventually, yielding the specification $\varphi := \Eventually m_1 \land \Eventually m_2$.

When trying to synthesize individual winning strategies for $p_1$ and $p_2$ separately, both synthesis tasks fail: while there exists a strategy for $p_i$ satisfying $\Eventually m_i$, a strategy for $p_i$ cannot influence variable $m_{1-i}$. Therefore, there is no strategy for $p_i$ that can ensure that $\Eventually m_{1-i}$ is satisfied for every input sequence.
However, since both processes build a system, the other process is most likely not completely adversarial; in fact, it even tries to satisfy $\varphi$ itself. Hence, it suffices to synthesis a strategy for $p_i$ that is \emph{as good as possible}: the other process will not produce a sequence that enforces a violation $\Eventually m_{1-i}$ and therefore $\varphi$ will not be violated in the interplay of both processes.

A dominant strategy for $p_i$ is allowed to violate $\varphi$ in situations in which no other strategy would have satisfied $\varphi$ either. A strategy $s_i$ for $p_i$ that outputs $m_i$ in the very first time step is dominant: it clearly satisfies $\Eventually m_i$ and only violates $\Eventually m_{1-i}$ if the input sequence does not contain any $m_{1-i}$. But then no strategy for $p_i$ at all satisfies $\varphi$ since no strategy for $p_i$ can influence $m_{1-i}$. 
The parallel composition of the dominant strategies $s_1$ and $s_2$ is a strategy that outputs both~$m_1$ and $m_2$ in the very first time step and thus satisfies $\varphi$.

Yet, $s_i$ is not the only dominant strategy for $p_i$. A strategy $s'_i$ that only outputs $m_i$ after receiving the other processes' message $m_{1-i}$ is dominant as well: it violates $\Eventually m_i$ if $p_{1-i}$ never outputs $m_{1-i}$. But then $\Eventually m_{1-i}$ is violated as well and therefore $s'_i$ is allowed to violate $\Eventually m_i$.
The parallel composition of the dominant strategies $s'_1$ and~$s'_2$ is a strategy that neither outputs $m_1$ nor $m_2$ at any point in time since $p_1$ and $p_2$ wait for each other indefinitely. Hence, it violates $\varphi$, while there are other strategies, \eg, $s_1 \pc s_2$, that satisfy~$\varphi$.

Hence, for liveness specifications, the parallel composition of two dominant strategies is not guarantees to be dominant. If we do not only take the satisfaction of $\varphi$ into account when considering dominance but also how \emph{fast} a strategy satisfies $\varphi$, we can exclude strategies whose progress unnecessarily depends on the behavior of another process from the possible strategies.
In this paper, we introduce a process requirement, \ddominance, that, similar to classical dominance, allows for \emph{best effort} strategies but utilizes a progress measure based on the universal co-Büchi automaton representing the specification that prioritizes fast strategies.
Hence, $s'_1$ and $s'_2$ are not \ddominant for $p_1$ and $p_2$. The strategies $s_1$ and $s_2$ that output $m_1$ and $m_2$ independent of the respective other process, however, are \ddominant. In this way, the parallel composition of \ddominant strategies is guaranteed to be dominant as well.

\Ddominance excludes the aforementioned strategies that wait indefinitely for each other from the set of possible strategies for $p_1$ and $p_2$. The strategies that output $r$ and $d$ independent of the respective other process, however, are \ddominant. In this way, the parallel composition of \ddominant strategies of $\controller$ and $\sensor$ is guaranteed to be dominant.

%Consider a distributed system for coordinating and executing measurements. The system consists of a controller $\controller$ and $k$ sensors $\sensor_1, \dots, \sensor_k$. The controller requests data from sensor $\sensor_i$ with variables $r_i$. The sensors provide data with variables $d_1, \dots, d_k$. While all $r_j$ with $1 \leq j \leq k$ are output variables of $\controller$, all $d_i$ with $1 \leq j \leq k$ are input variables of $\controller$. For sensor $\sensor_i$, $r_i$ is an input variable, while $d_i$ is an output variable.
%The sensors are required to answer a request for data eventually: $\varphi_\mathit{data} := \bigwedge_{1 \leq j \leq k} \Globally (r_i \rightarrow \Eventually d_i)$. Moreover, the controller is required to never cease to send data requests to the sensors, \ie, it sends requests infinitely often: $\varphi_\mathit{req} := \bigwedge_{1 \leq j \leq k} \Globally \Eventually r_i$.
%There can be further constraints on when the controller is required to send requests and on when the sensors are able to provide date. For simplicity, however, we assume that these are the only constraints and that the system only contains a single sensor $\sensor$. Thus, there is only a single request variable $r$ and only a single data variable $d$. The overall specification is then given by $\varphi := \Globally (r \rightarrow \Eventually d) \land \Globally \Eventually r$.
%
%When trying to synthesize winning strategies for $\controller$ and $\sensor$ for $\varphi$ separately, the synthesis task for $\controller$ fails: A strategy needs to output $r$ infinitely often. Yet, no matter at which point in time it outputs $r$, the adversarial sensor -- it is adversarial since we synthesize strategies for the processes individually -- might never provide data after this point in time, yielding a violation of $\varphi$.
%However, since $\controller$ and $\sensor$ build a system, $\sensor$ is not completely adversarial; in fact, it even tries to satisfy $\varphi$ as well. Hence, it suffices to synthesize a strategy for $\controller$ that is \emph{as good as possible}: $\sensor$ will not produce the sequence that enforces a violation of~$\varphi$ and therefore this violation will not occur in the interplay of $\controller$ and $\sensor$.
%
%A dominant strategy for $\controller$ is allowed to violate $\varphi$ in situations in which no other strategy would have satisfied $\varphi$ either. A strategy for $\controller$ that outputs $r$ infinitely often is dominant: it clearly satisfies the second conjunct of $\varphi$ and the first conjunct can only be not satisfied if the sensor ceases to transmit data at some point in time. But then no other strategy for $\controller$ would satisfy $\varphi$ either.
%A strategy for $\sensor$ that outputs $d$ infinitely often is dominant for $\varphi$: it is winning for the first conjunct of $\varphi$ and $\sensor$ cannot influence the second conjunct.
%The parallel composition of those two strategies then indeed yields a system that satisfies $\varphi$.
%
%However, the outlined strategies are not the only dominant strategies for~$\controller$ and $\sensor$.
%Another dominant strategy for $\controller$ is to send one initial request and then to only output $r$ once $\sensor$ outputted $d$. If $\sensor$ ceases to transmit data at some point in time, this strategy for $\controller$ does not satisfy $\Globally \Eventually r$. However, no controller strategy can then satisfy the first conjunct of $\varphi$ either. Hence, $\controller$ is allowed to violate $\varphi$ in this situation.
%Similarly, it is dominant for $\sensor$ to not transmit data directly after a request but only after a second request has been posed.
%The parallel composition of those strategies is not dominant: after an initial request, it neither outputs $r$ nor $d$ anymore since both processes wait for the other one indefinitely. Thus, it violates $\varphi$, while there clearly is a strategy for the whole system that satisfies $\varphi$, namely one that outputs both $r$ and $d$ infinitely often.
%
%
%If we do not only take satisfaction of $\varphi$ into account when considering dominance but also how \emph{fast} a strategy satisfies $\varphi$, strategies whose progress unnecessarily depends on progress of the other process can be excluded. In this paper, we introduce a winning condition for strategies, \ddominance, that, similar to dominance, allows for ``best effort'' strategies, but utilizes a progress measure based on the universal co-Büchi automaton representing the specification that prioritizes fast strategies. \Ddominance excludes the aforementioned strategies that wait indefinitely for each other from the set of possible strategies for $\controller$ and $\sensor$. The strategies that output $r$ and $d$ independent of the respective other process, however, are \ddominant. In this way, the parallel composition of \ddominant strategies of $\controller$ and $\sensor$ is guaranteed to be dominant.\todo{Potentiell neu schreiben}
